A projector-based convergence proof of the Ginelli algorithm for covariant Lyapunov vectors

Linear perturbations of solutions of dynamical systems exhibit different asymptotic growth rates, which are naturally characterized by so-called covariant Lyapunov vectors (CLVs). Due to an increased interest of CLVs in applications, several algorithms were developed to compute them. The Ginelli algorithm is among the most commonly used. Although several properties of the algorithm have been analyzed, there exists no mathematically rigorous convergence proof yet. In this article we extend existing approaches in order to construct a projector-based convergence proof of Ginelli's algorithm. One of the main ingredients will be an asymptotic characterization of CLVs via the Multiplicative Ergodic Theorem. In the proof, we keep a rather general setting allowing even for degenerate Lyapunov spectra.

==> Evolution.tex <==
\section{Ginelli's Algorithm}\label{sectionGinellisAlgorithm}
	Understanding long term behavior of solutions can prove to be a challenging task due to nonlinearity of the underlying system. However, locally, around a reference solution the problem becomes a lot easier. Instead of the full non-linear dynamics, it may be sufficient to only regard the tangent linear model along the reference solution for a qualitative analysis. Properties such as directions of different asymptotic growth rates can be computed via Ginelli's algorithm.\\

\subsection{Setting}\label{subsectionSetting}
	Since we want to cover as many applications for Ginelli's algorithm as possible, we do not specify a type of state space or system. Instead, we assume a non-empty set $\Omega=\left\{\theta_t\omega_0\ |\ t\in\mathbb{T}\right\}$ to be the abstract orbit of our state of interest $\omega_0$ respective to the flow $(\theta_t)_{t\in\mathbb{T}}$. Here, $\theta_t:\Omega\to\Omega$ represents the time-$t$-flow on our orbit. The flow should satisfy $\theta_0=\textnormal{id}_{\Omega}$ and $\theta_{s+t}=\theta_s\theta_t$. Remaining information of the linear model is encoded in a cocycle $\Phi(t,\omega)$ assigning a time-step $t$ and a state $\omega$ to the linear propagator on tangent space from $\omega$ to $\theta_t\omega$.
	
	\begin{definition}\label{definitionCocycle}
		A map $\Phi:\mathbb{T}\times\Omega\to\real^{d\times d}$ is called a \emph{(linear) cocycle (over $\theta$)} if
		\begin{enumerate}
			\item $\Phi(0,\omega)=\textnormal{id}$
			\item $\Phi(s+t,\omega)=\Phi(s,\theta_t\omega)\Phi(t,\omega)$
		\end{enumerate}
		are satisfies for all $s,t\in\mathbb{T}$ and $\omega\in\Omega$.
	\end{definition}
	Since $\mathbb{T}$ is two-sided, the cocycle is point-wise invertible with inverse
	\begin{equation*}
		\Phi(t,\omega)^{-1}=\Phi(-t,\theta_t\omega).
	\end{equation*}
	The Multiplicative Ergodic Theorem of Oseledets \autocite{Oseledets1968} is not only necessary to describe existence of CLVs, but will play a crucial role in our convergence proof. We state a deterministic version found in \autocite{Arnold1998}. It assumes that changes during a short time-step do not matter on the exponential scale and, furthermore, that expansion rates of different volumes are well-defined and do not exceed the exponential scale.
	\begin{proposition}[Deterministic MET]\label{propositionDeterministicMET}
		Let $\Phi$ be a cocycle satisfying
		\begin{equation*}
			\lambda\left(\sup_{s\in[0,1]\cap\mathbb{T}}\|\Phi(s,\theta_t\omega_0)^{\pm 1}\|\right)\leq 0
		\end{equation*}
		and assume that 
		\begin{equation*}
			\lim_{t\to\infty}\frac{1}{t}\log\|\wedge^i\Phi(t,\omega_0)\|\in\real\cup\{-\infty\}
		\end{equation*}
		exists for all orders of the wedge product of $\Phi(t,\omega_0)$. Then, there is a Lyapunov spectrum with a corresponding filtration capturing subspaces of different growth rates:
		\begin{enumerate}
			\item The \emph{Lyapunov spectrum} consists of \emph{Lyapunov exponents} (LEs)
			\begin{equation*}
				-\infty\leq\lambda_p<\dots<\lambda_1<\infty,
			\end{equation*}
			which are the distinct limits of singular values, together with degeneracies $d_1+\dots+d_p=d$:
			\begin{equation}\label{equationSingularValuesLEs}
				\forall i:\ \forall k=1,\dots,d_i:\ \lambda_{i}=\lim_{t\to\infty}\frac{1}{t}\log\sigma_{i_k}\left(\Phi(t,\omega_0)\right)
			\end{equation}
			\item There is a filtration
			\begin{equation*}
				\{0\}=:V_{p+1}\subset V_p\subset \dots\subset V_1=\real^d
			\end{equation*}
			given by subspaces
			\begin{equation*}
				V_i:=\left\{x\in\real^d\ \left|\ \lim_{t\to\infty}\frac{1}{t}\log\|\Phi(t,\omega_0)x\|\leq\lambda_i \right.\right\}.
			\end{equation*}
			Limits in the definition of $V_i$ exist for each $x\in\real^d$ and take values in $\{\lambda_1,\dots,\lambda_p\}$. Moreover, it holds
			\begin{equation*}
				\dim V_i-\dim V_{i+1}=d_i.
			\end{equation*}
		\end{enumerate}
	\end{proposition}
	The proposition only requires one-sided time and an invertible cocycle to provide the Lyapunov spectrum and filtration at state $\omega_0$ of the orbit. However, since we assumed two-sided time, we immediately get the existence of those quantities for all states along the orbit.
	\begin{corollary}\label{corollaryMETWholeOrbit}
		In the setting of proposition \textnormal{\ref{propositionDeterministicMET}} the Lyapunov spectrum and filtration are defined for all $\omega\in\Omega$. Furthermore, $p(\omega)$, $\lambda_i(\omega)$ and $d_i(\omega)$ are independent of $\omega$, and the filtration changes in a covariant way:
		\begin{equation*}
			\Phi(t,\omega)V_i(\omega)=V_i(\theta_t\omega)
		\end{equation*}
	\end{corollary}
	\begin{proof}
		The first assumption of proposition \ref{propositionDeterministicMET} is trivially satisfied if we replace $\omega_0$ by $\omega=\theta_u\omega_0$. To prove the second assumption we use the following properties for the wedge product of $A,B\in\real^{d\times d}$, which can be found in \autocite{Arnold1998}:
		\begin{enumerate}
			\item $\|\wedge^iA\|=\sigma_1(A)\dots\sigma_i(A)$
			\item $\|\wedge^i(AB)\|\leq\|\wedge^iA\|\|\wedge^iB\|$
		\end{enumerate}
		Now, the existence of
		\begin{equation*}
			\lim_{t\to\infty}\frac{1}{t}\log\|\wedge^i\Phi(t,\theta_u\omega_0)\|<\infty
		\end{equation*}
		follows due to the cocycle property:
		\begin{align*}
			&\left(\frac{t+u}{t}\right)\left(\frac{1}{t+u}\log\|\wedge^i\Phi(t+u,\omega_0)\|\right)-\frac{1}{t}\log\|\wedge^i\Phi(u,\omega_0)\|\\
			&\hspace{1em}\leq\frac{1}{t}\log\|\wedge^i\Phi(t,\theta_u\omega_0)\|\\
			&\hspace{1em}\leq\left(\frac{t+u}{t}\right)\left(\frac{1}{t+u}\log\|\wedge^i\Phi(t+u,\omega_0)\|\right)+\frac{1}{t}\log\|\wedge^i\Phi(-u,\theta_u\omega_0)\|
		\end{align*}
		Thus, the proposition gives us the existence of a Lyapunov spectrum and filtration at state $\omega$. In particular, limits of singular values for $\omega$ and $\omega_0$ do not differ on the exponential scale. Hence, the remaining statements of corollary \ref{corollaryMETWholeOrbit} follow.
	\end{proof}
	Similar statements can be derived for the time-reversed cocycle $\Phi^-(t,\omega):=\Phi(-t,\omega)$ over the time-reversed flow $\theta^-_t:=\theta_{-t}$. We denote its Lyapunov spectrum by $(\lambda_{i}^-,d_i^-)_{i=1,\dots,p^-}$ and the corresponding filtration spaces by $V_i^-(\omega)$.\\
	
	In order to define a covariant splitting of the tangent space that captures asymptotic growth rates in forward and backward time, we require two additional assumptions:
	\begin{enumerate}
		\item $(d^-)=(d)^r$ and $\left(\lambda^-\right)=\left(-\lambda\right)^r$
		\item $V_{i+1}(\omega_0)\cap V_{p+1-i}^-(\omega_0)=\{0\}$
	\end{enumerate}
	A direct consequence is that LEs are finite. For convenience sake, we set $\lambda_0:=\infty$ and $\lambda_{p+1}:=-\infty$.\\
	
	Assuming the above, we get the existence of Oseledets spaces characterizing asymptotic dynamics.
	\begin{proposition}\label{propositionOseledetsSpaces}
		There is a splitting $\real^d=E_1(\omega)\oplus\dots\oplus E_p(\omega)$ of the tangent space into so-called \emph{Oseledets spaces}
		\begin{equation}\label{equationOseledetsSpacesIntersection}
			E_i(\omega):=V_i(\omega)\cap V_{p+1-i}^-(\omega).
		\end{equation}
		Furthermore, Oseledets spaces can be characterized via
		\begin{equation}\label{equationOseledetsSpacesAsymptotics}
			x\in E_i(\omega)\setminus\{0\}\iff \lim_{t\to\pm\infty}\frac{1}{|t|}\log\|\Phi(t,\omega)x\|=\pm\lambda_i,
		\end{equation}
		are covariant 
		\begin{equation*}
			\Phi(t,\omega)E_i(\omega)=E_i(\theta_t\omega)
		\end{equation*}
		and satisfy $\dim E_i(\omega)=d_i$.
	\end{proposition}
	\begin{proof}
		The proof is purely algebraic and can be found along the lines of the proof of the MET for two-sided time in \autocite{Arnold1998}.
	\end{proof}
	For a random dynamical system satisfying some integrability condition, it is shown in \autocite{Arnold1998} that the cocycle along almost all orbits of the system admits an Oseledets splitting. Moreover, in an ergodic setting the Lyapunov spectrum for almost all orbits coincides. Therefore, in applications it is often conveniently assumed that the underlying system is ergodic at least near an interesting structure.\footnote{For example, see the concept of SRB-measures for attractors \autocite{Bowen1975}.} Via CLVs one hopes to better understand the local flow around this structure.
	\begin{definition}\label{definitionCLVs}
		Normalized basis vectors, which are covariant and chosen subject to the Oseledets splitting for each $\omega\in\Omega$, are called \emph{covariant Lyapunov vectors (CLVs)}.
	\end{definition}
	 CLVs represent directions of different asymptotic growth rates\footnote{Aside from asymptotic growth, the angle between CLVs can be used as a measure of hyperbolicity (see, e.g., \autocite{Conti2017}).} by ($\ref{equationOseledetsSpacesAsymptotics}$). However, they are only uniquely defined (up to sign) for non-degenerate Lyapunov spectra.
	
	
\subsection{The Algorithm}\label{subsectionTheAlgorithm}
	The Ginelli algorithm \autocite{Ginelli2007, Ginelli2013} computes Oseledets spaces (or CLVs) for a given cocycle by using its asymptotic characterization (\ref{equationOseledetsSpacesAsymptotics}). The main idea is that every vector with a non-zero $E_1$-part will approach $E_1$ asymptotically, since its $E_1$-component has the biggest exponential growth rate. More abstractly, almost all $(d_1+\dots+d_i)$-dimensional subspaces align with $E_1\oplus\dots\oplus E_i$, the fastest expanding (or slowest contracting) subspace of the corresponding dimension, in forward time.\\
	Reversing time, we are able to extract the slowest expanding (or fastest contracting) subspace. In particular, almost all $d_i$-dimensional subspaces of $E_1\oplus \dots\oplus E_i$ will align with $E_i$ in backward time.\\
	 
	Taking these traits into consideration, the abstract formalism of Ginelli's algorithm is as follows:\\
	
	\textbf{Ginelli Algorithm}\\
	\begin{enumerate}
		\item[1.1.] Randomly choose a basis $(b)$ of the tangent space at a past state $\theta_{-t_1}\omega_0$ and propagate it forward until $\omega_0$. If the propagation time $t_1$ is chosen large enough, we expect $\Phi(t_1,\theta_{-t_1}\omega_0)\overline{U}_i^{(b)}=\overline{U}_i^{(\Phi(t_1,\theta_{-t_1}\omega_0)b)}$ to be a good approximation to $E_1(\omega_0)\oplus\dots\oplus E_i(\omega_0)$.
		\item[1.2.] Continue forward propagation until a state $\theta_{t_2}\omega_0$ is reached. This state should be far enough in the future, so that we have a sufficiently good approximation to $E_1\oplus\dots\oplus E_i$ on a long enough time-frame for the second phase.
		\item[2.] For each $i$, randomly choose $d_i$ vectors $b_{i_1}',\dots,b_{i_{d_i}}'$ in $\overline{U}_i^{(\Phi(t_1+t_2,\theta_{-t_1}\omega_0)b)}\approx E_1(\theta_{t_2}\omega_0)\oplus\dots\oplus E_i(\theta_{t_2}\omega_0)$ and propagate them backward until $\omega_0$. The evolved subspace $U_i^{(\Phi(-t_2,\theta_{t_2}\omega_0)b')}$ is our approximation to $E_i(\omega_0)$. 
	\end{enumerate}
	Since we propagate vectors forward, we call steps 1.1 and 1.2 \emph{forward phase}\footnote{Numerically, it makes sense to apply the cocycle in small time-steps and orthonormalize the basis in-between. Otherwise computations become singular, as all vectors will collapse onto the first Oseledets space. However, analytically, proposition \ref{propositionGramSchmidtInBetweenCocylce} tells us that there is no difference in applying the Gram-Schmidt procedure between every step or just once at the end.}, and by the same reasoning step 2 is called \emph{backward phase}\footnote{Here, assuming the Lyapunov spectrum is known, it appears numerically advantageous to orthonormalize $b_{i_1}',\dots,b_{i_{d_i}}'$ in between propagation steps.}.
	\begin{figure}[H]
		\makebox[\textwidth][c]{\includegraphics[width=1.083\linewidth]{figures/Ginelli.pdf}}
		\begin{center}
			\title{schematic picture of the Ginelli algorithm}
		\end{center}
	\end{figure}
	
	The asymptotic expansion rate $(\lambda_1+\dots+\lambda_{i})$ of $E_1\oplus\dots\oplus E_i$ is usually computed as a byproduct in the forward phase of the algorithm. Using this information, we can derive the Lyapunov spectrum.\footnote{This concept was already used in 1980 by Benettin \autocite{Benettin1980Part1,Benettin1980Part2} to compute the Lyapunov spectrum. Therefore, subsequent application of the cocycle and orthonormalization is sometimes called a \emph{Benettin step}.}\\
	
	We provide a convergence proof of the whole algorithm as $\min(t_1,t_2)\to\infty$ in chapter \ref{sectionConvergence}. The convergence speed turns out to be exponential in relation to the minimum distance of LEs. Furthermore, the kind of convergence differs between discrete and continuous time. The discrete version with $t_1,t_2\in\natural$ converges for almost all initial tuples, whereas the continuous version with $t_1,t_2\in\real_{> 0}$ only converges in measure.\\
	
	Next, we present what might happen in the forward phase for some exemplary cocycles. We start with a very simple example that demonstrates how almost all vectors should evolve in a non-degenerate setting.\\
	
	\begin{example}[diagonal cocylce]\label{exampleDiagonalCocycle}
		Assume $\Omega=\{\omega_0\}$ with trivial flow $\theta_t\omega_0=\omega_0$. For given $\lambda_1>\dots>\lambda_p$, define $D:=\textnormal{diag}\left(e^{\lambda_1},\dots,e^{\lambda_p}\right)$. Then, $\Phi(t,\omega_0):=D^t$ is a cocycle and the CLVs (at $\omega_0$) coincide with the standard basis $(e)$ of $\real^d$.\\
		
		Now, fix a vector $b_1\in\real^d$ with $|\langle b_1,e_1\rangle|>0$. We have
		\begin{equation*}
			\langle D^t b_1,e_i\rangle=\langle b_1,e_i\rangle e^{t\lambda_i}.
		\end{equation*}
		Thus, we compute
		\begin{equation*}
			\left|\left\langle\frac{D^tb_1}{\|D^tb_1\|},e_i\right\rangle\right|^2=\frac{|\langle b_1,e_i\rangle|^2 e^{2t\lambda_i}}{\sum_j |\langle b_1,e_j\rangle|^2 e^{2t\lambda_j}}=\frac{|\langle b_1,e_i\rangle|^2 e^{-2t|\lambda_1-\lambda_i|}}{\sum_j |\langle b_1,e_j\rangle|^2 e^{-2t|\lambda_1-\lambda_j|}}.
		\end{equation*}
		The last nominator takes values between $|\langle b_1,e_1\rangle|^2$ and $\|b_1\|^2$. In particular, it can be treated as a positive constant for the Lyapunov index notation:
		\begin{align*}
			\lambda\left(d\left(\overline{U}_1^{(D^tb)},\overline{U}_1^{(e)}\right)\right)&=\lambda\left(\|\left(I-\overline{P}_1^{(e)}\right)\overline{P}_1^{(D^tb)}\|\right)\\
			&=\lambda\left(\sum_{i\neq 1}\left|\left\langle\frac{D^tb_1}{\|D^tb_1\|},e_i\right\rangle\right|\right)\\
			&\leq \max_{i\neq 1} \lambda\left(\left|\left\langle\frac{D^tb_1}{\|D^tb_1\|},e_i\right\rangle\right|\right)\\
			&\leq \max_{i\neq 1}-|\lambda_1-\lambda_i|\\
			&=-|\lambda_1-\lambda_2|
		\end{align*}
		In general it holds
		\begin{equation*}
			\lambda\left(d\left(\overline{U}_i^{(D^tb)},\overline{U}_i^{(e)}\right)\right)\leq -|\lambda_{i}-\lambda_{i+1}|
		\end{equation*}
		for all tuples $(b)$ that are admissible w.r.t. $(e)$. We will show that this is true for arbitrary cocycles satisfying the assumptions in section \textnormal{\ref{subsectionSetting}}.
	\end{example}
	
	Ginelli's algorithm starts with a random choice of initial vectors to prevent non-admissible configuration. One such configuration would be the unlikely case where the first vector lies in the second Oseledets space. As Oseledets spaces are covariant, the first vector will stay inside the second Oseledets space when propagated. Consequently, the algorithm does not yield a good approximation.\\
	
	The next example shows that all vectors might be non-admissible when initiated at a wrong time in the continuous version of Ginelli's algorithm.
	
	\begin{example}[rotating Oseledets spaces]\label{exampleRotatingOseledetsSpaces}
		Let $\Omega:=S^1\cong\qspace{\real}{\integer}$ be a periodic orbit with normalized flow $\theta_t\omega:=\omega+t$. Furthermore, let $R:\real\to SO(2)$ be the parametrization of $SO(2)$ by $2\times 2$ rotation matrices
		\begin{equation*}
		R(\omega):=\begin{pmatrix}
		\cos(2\pi\omega) & -\sin(2\pi\omega)\\
		\sin(2\pi\omega) & \cos(2\pi\omega)
		\end{pmatrix},
		\end{equation*}
		so that $R(0)=R(1)=I$ and $R(s+t)=R(s)R(t)$. Moreover, we set $D:=\textnormal{diag}\left(e^{\lambda_1},e^{\lambda_2}\right)$ for some $\lambda_1>\lambda_2$, and define the cocycle to be
		\begin{equation*}
		\Phi(t,\omega):=R(\theta_t\omega)D^tR(-\omega).
		\end{equation*}
		One readily checks that $\Phi(t,\omega)$ indeed is a cocycle over $\theta$.\\
		
		We use the characterization of Oseledets spaces via asymptotic growth rates:
		\begin{align*}
		\lim\limits_{t\to\pm\infty}\frac{1}{t}\log\|\Phi(t,\omega)\cdot R(\omega)\begin{pmatrix} x_1 \\ x_2 \end{pmatrix}\|&=
		\begin{cases}
		\lambda_1 &x_1\neq 0\text{ and }x_2=0 \\
		\lambda_2 &x_1=0\text{ and }x_2\neq 0
		\end{cases}\\
		\Rightarrow\hspace{1em}E_1(\omega)=\textnormal{span}\left(R(\omega)\begin{pmatrix} 1 \\ 0 \end{pmatrix}\right)\hspace{1em}&\text{and}\hspace{1em}E_2(\omega)=\textnormal{span}\left(R(\omega)\begin{pmatrix} 0 \\ 1 \end{pmatrix}\right)
		\end{align*}
		In particular, both Oseledets spaces are rotating uniformly with varying $\omega$. Hence, for any fixed vector $b_1\in\real^2$ and $T>0$, we find $t_1\in\real_{>0}$ bigger than $T$ with $b_1\in E_2(\theta_{-t_1}\omega)$, which implies that the continuous version of Ginelli's algorithm does not converge for any fixed choice of $b_1$. Instead, we will prove convergence in measure for the continuous case later on.\\
		In the discrete case, however, the set $\bigcup_{t_1\in\natural}E_2(\theta_{-t_1}\omega)$ has Lebesgue-measure zero indicating that convergence for almost all initial tuples is still possible.
	\end{example}
	Setting $D=\textnormal{diag}(e^{\lambda_1},e^{\lambda_1})$ in the previous example yields a trivial Oseledets space $E_1(\omega)=\real^2$ with inner rotation. In general, Oseledets spaces can have complicated internal dynamics that prevent propagated vectors from converging. Additionally, we already remarked that CLVs are not uniquely defined in presence of degeneracies. Therefore, objects of interest should not be the propagated vectors themselves but the spaces spanned by them subject to degeneracies.\footnote{Practically speaking, degeneracies can be derived from growth rates of propagated vectors during the forward phase. They might be forced by symmetries (e.g. equivariant systems), whereas, for some classes of systems degenerate scenarios are the exception \autocite{Arnold1999}.}\\
	
	As a closing remark for this chapter, we would like to mention that there are several other recently developed algorithms, see \autocite{Froyland2013,Kuptsov2012,Wolfe2007}, some of which can be treated in a similar fashion to Ginelli's algorithm with the tools developed here.\\	
	
	
%	other possible examples: RDS via MET of \autocite{Arnold1998}; equivariant ODEs
	
%	\begin{example}[equivariant ODEs]\label{exampleEquivariantODEs}
%		Let $\dot{\omega}=f(\omega)$ be a smooth autonomous ODE defined on some open subset $\Omega\subset\real^d$ with globally defined flow $\left(\theta(t)\right)_{t\in\real}$ on $\Omega$. Moreover, assume that the flow preserves some probability measure $\mathbb{P}$ on $\Omega$. We naturally get a cocycle over $\theta$ by linearizing the flow: $\Phi(t,\omega):=D_{\omega}(\theta(t))(\omega)$. If the cocycle satisfies the integrability condition of the MET, then we have the existence of a flow-invariant set $\tilde{\Omega}\subset\Omega$ of full $\mathbb{P}$-measure on which the Oseledets spaces are defined.\\
%		Now, look at a setting where $f$ is equivariant under the action of some group $\Gamma\subset Gl(d,\real)$:
%		\begin{equation*}
%		\forall \gamma\in\Gamma\ :\ f(\gamma\cdot\omega)=\gamma\cdot f(\omega)
%		\end{equation*}
%		It follows that $\theta(t)$ commutes with the $\Gamma$-action for each $t\in\real$. Moreover, the cocycle $\Phi$ satisfies
%		\begin{equation*}
%		\forall \gamma,t,\omega\ :\ \Phi(t,\omega)=\gamma^{-1}\cdot\Phi(t,\gamma\cdot\omega)\cdot\gamma.
%		\end{equation*}
%		In particular, for $\omega\in\tilde{\Omega}\cap \textnormal{Fix}(\Gamma)$, we get
%		\begin{equation*}
%		\lambda(\omega,x)=\lim_{t\to\infty}\frac{1}{t}\log \|\Phi(t,\omega)x\|\leq\lim_{t\to\infty}\frac{1}{t}\log \|\Phi(t,\omega)\gamma\cdot x\|=\lambda(\omega,\gamma\cdot x).
%		\end{equation*}
%		Interchanging $x$ by $\gamma\cdot x$ and $\gamma$ by $\gamma^{-1}$ yields equality of $\lambda(\omega,x)$ and $\lambda(\omega,\gamma\cdot x)$. Hence, the filtration spaces $V_i(\omega)$ from the MET are invariant under the group action. By repetition of the same argument for the reversed cocycle, we get invariance of the filtration spaces $V_i^-(\omega)$. As Oseledets spaces are just intersections of those spaces, they are also invariant under the action of $\Gamma$. This can force Oseledets spaces to have higher dimensions and, hence, induces degenerate Lyapunov spectra.
%	\end{example}
